Acceleration of SVRG and Katyusha X by Inexact Preconditioning

Empirical risk minimization is an important class of optimization problems with many popular machine learning applications, and stochastic variance reduction methods are popular choices for solving them. Among these methods, SVRG and Katyusha X (a Nesterov accelerated SVRG) achieve fast convergence without substantial memory requirement. In this paper, we propose to accelerate these two algorithms by \textit{inexact preconditioning}, the proposed methods employ \textit{fixed} preconditioners, although the subproblem in each epoch becomes harder, it suffices to apply \textit{fixed} number of simple subroutines to solve it inexactly, without losing the overall convergence. As a result, this inexact preconditioning strategy gives provably better iteration complexity and gradient complexity over SVRG and Katyusha X. We also allow each function in the finite sum to be nonconvex while the sum is strongly convex. In our numerical experiments, we observe an on average $8\times$ speedup on the number of iterations and $7\times$ speedup on runtime.

==> FancyArticlePackages.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    ~~~ Fancy Article Packages ~~~    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% A useful and fancy collection of Latex packages
% Describes the function of each package briefly.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Font packages: input, output, etc.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}

%Latin modern font
\usepackage{lmodern}

%embolden text
\usepackage{bm}

%colored fonts
\usepackage{color}

%Stretches and shrinks fonts to fit on line a little better
\usepackage{microtype}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Standard AMS and math packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%amsmath: miscellaneous enhancements for mathematical documents.
\usepackage{amsmath}

%amsthm: Package for theorem-like structures: theorem, lemma, proof, corollary, etc.
\usepackage{amsthm}

%amssymb: extension of symbol collection.
\usepackage{amssymb}

%mathtools: Extends and fixes deficiencies in amsmath
\usepackage[showonlyrefs]{mathtools}
%showonlyrefs: Only show equation numbers when cross referenced somewhere

%array and tabular environment
\usepackage{array}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Miscellaneous:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%authblk: author/affiliation and footnote style authors.
\usepackage{authblk}

%Paper size and page margins
\usepackage{geometry}

%Fancy headers on every page: Section and subsection on left and right respectively
%Fancy headers on every page: Section and subsection on left and right respectively
%\usepackage{fancyhdr, blindtext}
%\newcommand{\changefont}{\fontsize{7}{9}\selectfont}
%\fancyhf{}
%\fancyhead[R]{\changefont \slshape \rightmark} %section
%\fancyhead[L]{\changefont \slshape \textbf{\leftmark}} %chapter
%\fancyfoot[C]{\changefont \thepage} %footer
%\pagestyle{fancy}

%Fixed-length columns with L, C, R alignment.
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

%Todonotes package: Useful for commenting in collaboration
\usepackage[colorinlistoftodos]{todonotes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Referencing and bibliography
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%NOTE: Bibliography package has been removed since this often needs to be changed, and certain biliography settings can only be set at load time. See article template.
%biblatex: Bibliography package
%biber: Recommended backend
%ieee: Nice looking style
%url = false: Suppresses URLs for non websites. Doesn't seem to work for arXiv.
%\usepackage[backend=biber,style=ieee]{biblatex}

%Hyperref: set up cross reference and citation links
%Also creates bookmarks for sections, subsections, etc.
\usepackage{hyperref}
\hypersetup{colorlinks=true, linkcolor=blue, citecolor=blue, urlcolor=blue,bookmarksnumbered,bookmarksdepth=3}

%Cleveref: Allows labeled references. E.g. "Theorem 10" instead of "10".
%Find this package in the FancyMathAndTheoremEnvironments.tex file. Needs to be here for package ordering reasons.
%\cref: Gives short form. E.g. Cor. 11, Defn. 24
%\Cref: Gives long form. E.g. Theorem 13, Definition 8
